Searching for P- and CP- odd effects in heavy ion collisions

In this thesis we study the possibility that QCD breaks parity at high temperatures and densities, a scenario that may be tested in heavy ion collisions. Analytical studies with effective models suggest that QCD may break parity in dense systems. Besides, P- and CP- odd bubbles may appear in a finite volume due to local large topological fluctuations in a hot medium. The last effect may be treated in a quasi-equilibrium description by means of a non-trivial axial chemical potential. We consider the 'two flavour' Nambu--Jona-Lasinio model in the presence of a vector and an axial external chemical potentials and study the phase structure of the model at zero temperature. These magnitudes could trigger a phase where parity could be broken in QCD. Analogies and differences with the expected behaviour in QCD are discussed besides the limitations of the model. We also consider the low energy realization of QCD in terms of mesons when an axial chemical potential is present. The eigenstates of strong interactions do not have a definite parity and interactions that would otherwise be forbidden compete with the familiar ones. We focus on scalars and pseudoscalars that are described by a generalized linear sigma model. Finally, we investigate how local parity breaking may affect vector physics. A modified dispersion relation is derived for the lightest vector mesons rho and omega. This effect predicts a natural overproduction of lepton pairs in the vicinity of the rho-omega resonance peak as well as a polarization asymmetry around this peak. The dilepton excess seems relevant to explain the anomalous dielectron yield quoted by PHENIX/STAR. We present a detailed analysis of the angular distribution associated to the lepton pairs created from these mesons searching for polarization dependencies. Two angular variables are found to carry the main information related to the parity-breaking effect.

==> CHANGELOG <==
caption package
===============

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added


bicaption package
=================

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added


ltcaption package
=================

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator


subcaption package
==================

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption


newfloat package
================

v1.0 (2011/10/30)
- 1st published version

v1.1 (2013/04/27)
- New command \PrepareListOf


totalcount package
==================

v1.0 (2008/03/09)
- 1st published version



==> Latex/Classes/anyfontsize/README <==
anyfontsize.sty is a LaTeX2e package that lets the user select any 
font size (via e.g. \fontsize{...}{...}\selectfont), even those 
sizes that are not listed in the .fd file. If such a size is requested, 
LaTeX will search the nearest listed size, and anyfontsize will scale 
that font to the requested size. For a similar functionality that 
works only for the CM fonts, try the type1cm.sty package, or, even 
better, use the new Latin Modern (LM) fonts, which are available at 
any size.

License type: lppl


==> Latex/Classes/urlbst <==
#! /usr/bin/env perl
#
# Usage: ./urlbst.pl [--eprint] [--doi]
#    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]
#    [input-file [output-file]]
# If either input-file or output-file is omitted, they are replaced by
# stdin or stdout respectively.
#
# See http://purl.org/nxg/dist/urlbst for documentation
#
# $Id: urlbst.in,v 1.8 2007/03/26 17:21:56 norman Exp $

$version = '0.6';
($progname = $0) =~ s/.*\///;
$mymarker = "% $progname";
$mymarkerend = "% ...$progname to here";
$myurl = 'http://purl.org/nxg/dist/urlbst';


$infile = '-';
$outfile = '-';

$addeprints = 0;     # if true (nonzero) we add support for eprints
$eprintprefix = 'arXiv:';	# make these settable with --eprint? syntax?
$eprinturl = 'http://arxiv.org/abs/';

$adddoiresolver = '0';
$doiprefix = 'doi:';
$doiurl = 'http://dx.doi.org/';

$makehref = 0;
$availablestring = "Available from: ";
$inlinelinks = 0;

$Usage = "$progname [--eprint] [--doi]\n    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]\n    [--help] [input-file [output-file]]";

while ($#ARGV >= 0) {
    if ($ARGV[0] eq '--eprint') {
	$addeprints = 1;
    } elsif ($ARGV[0] eq '--doi') {
        $adddoiresolver = 1;
    } elsif ($ARGV[0] eq '--nohyperlinks') {
        $makehref = 0;
    } elsif ($ARGV[0] eq '--hypertex') {
	$makehref = 1;
    } elsif ($ARGV[0] eq '--hyperref') {
	$makehref = 2;
    } elsif ($ARGV[0] eq '--inlinelinks') {
        $inlinelinks = 1;
    } elsif ($ARGV[0] eq '--help') {
        print <<EOD;
urlbst version $version
    Usage: $Usage
      --eprint:       include support for `eprint' fields
      --doi:          include support for `doi' field
      --nohyperlinks  do not include active links anywhere
      --inlinelinks   add hyperlinks to entry titles
      --hypertex:     include HyperTeX-style hyperlink support
      --hyperref:     include {hyperref}-style hyperlink support
                      (generally better)
      --help:         print this help
    Input and output files may be given as `-' (default) to indicate stdin/out
EOD
        exit(0);
    } elsif ($ARGV[0] =~ /^-/) {
        die "Unrecognised option $ARGV[0]: Usage: $Usage\n";
    } elsif ($infile eq '-') {
	$infile = $ARGV[0];
    } elsif ($outfile eq '-') {
	$outfile = $ARGV[0];
    } else {
	die "Usage: $Usage\n";
    }
    shift(@ARGV);
}

if ($inlinelinks && $makehref == 0) {
    print <<'EOD';
Warning: --inlinelinks and --nohyperlinks were both specified (possibly
    implicitly).  That combination makes no sense, so I'll ignore
    --nohyperlinks and use --hyperref instead
EOD
    $makehref = 2;
}

$exitstatus = 0;		# success status

open (IN, "<$infile") || die "Can't open $infile to read";
open (OUT, ">$outfile") || die "Can't open $outfile to write";

# We have to make certain assumptions about the source files, in order
# to patch them at the correct places.  Specifically, we assume that
#
#   - there's a function init.state.consts
#
#   - ...and an output.nonnull which does the actual outputting, which
#         has the `usual' interface.
#
#   - we can replace
#           fin.entry
#       by
#           new.block
#           output.url    % the function which formats and displays any URL
#           fin.entry
#
#   - there is a function which handles the `article' entry type (this
#         will always be true)
#
#   - there is a function output.bibitem which is called at the
#         beginning of each entry type
#   - ...and one called fin.entry which is called at the end
#
# If the functions format.date, format.title or new.block are not defined (the
# former is not in apalike, for example, and the last is not in the
# AMS styles), then replacements are included in the output.
#
# All these assumptions are true of the standard files and, since most
# style files derive from them more or less directly, are true of most (?)
# other style files, too.
#
# There's some rather ugly Perl down here.  The parsing for
# brace-matching could probably do with being rewritten in places, to
# make it less ugly, and more robust.

print OUT "%%% Modification of BibTeX style file ", ($infile eq '-' ? '<stdin>' : $infile), "\n";
print OUT "%%% ... by $progname, version $version (marked with \"$mymarker\")\n%%% See <$myurl>\n";
print OUT "%%% Added webpage entry type, and url and lastchecked fields.\n";
print OUT "%%% Added eprint support.\n"   if ($addeprints);
print OUT "%%% Added DOI support.\n"      if ($adddoiresolver);
print OUT "%%% Added HyperTeX support.\n" if ($makehref == 1);
print OUT "%%% Added hyperref support.\n" if ($makehref == 2);
print OUT "%%% Original headers follow...\n\n";

$found{initconsts} = 0;
$found{outputnonnull} = 0;
$found{article} = 0;
$found{outputbibitem} = 0;
$found{finentry} = 0;
$found{formatdate} = 0;
$found{formattitle} = 0;
$found{newblock} = 0;

while (<IN>) {
    /^ *%/ && do {
        # Pass commented lines unchanged
        print OUT;
        next;
    };
    
    /^ *ENTRY/ && do {
	# Work through the list of entry types, finding what ones are there.
	# If we find a URL entry there already, object, since these edits
	# will mess things up.
	$line = $_;
	until ($line =~ /\{\s*(\w*)/) {
	    $line .= <IN>;
	}
	$bracematchtotal = 0;	# reset
	bracematcher($line);
	$line =~ /\{\s*(\w*)/;
	$found{'entry'.$1} = 1;
	print OUT $line;
	$line = <IN>;
	until (bracematcher($line) == 0) {
	    # XXX deal with multiple entries on one line
	    ($line =~ /^\s*(\w*)/) && ($found{'entry'.$1} = 1);
	    print OUT $line;
	    $line = <IN>;
	}
	if (defined($found{entryurl})) {
	    print STDERR "$progname: style file $infile already has URL entry!\n";
	    # print out the rest of the file, and give up
            print OUT $line;
	    while (<IN>) {
		print OUT;
	    }
	    $exitstatus = 1;
	    last;
	} else {
            print OUT "    eprint $mymarker\n    doi $mymarker\n    url $mymarker\n    lastchecked $mymarker\n";
	}
	print OUT $line;
	next;
    };

    /^ *FUNCTION *\{init\.state\.consts\}/ && do {
        # In the init.state.consts function, add an extra set of
        # constants at the beginning.  Also use this as the marker for
        # the place to add the init strings function.
        print OUT <<EOD;
STRINGS { urlintro eprinturl eprintprefix doiprefix doiurl openinlinelink closeinlinelink } $mymarker...
INTEGERS { hrefform inlinelinks makeinlinelink addeprints adddoiresolver }
% Following constants may be adjusted by hand, if desired
FUNCTION {init.urlbst.variables}
{
  "$availablestring" 'urlintro := % prefix before URL
  "$eprinturl" 'eprinturl := % prefix to make URL from eprint ref
  "$eprintprefix" 'eprintprefix := % text prefix printed before eprint ref
  "$doiurl" 'doiurl := % prefix to make URL from DOI
  "$doiprefix" 'doiprefix :=      % text prefix printed before DOI ref
  #$addeprints 'addeprints :=         % 0=no eprints; 1=include eprints
  #$adddoiresolver 'adddoiresolver :=     % 0=no DOI resolver; 1=include it
  #$makehref 'hrefform :=           % 0=no crossrefs; 1=hypertex xrefs; 2=hyperref refs
  #$inlinelinks 'inlinelinks :=        % 0=URLs explicit; 1=URLs attached to titles
  % the following are internal state variables, not config constants
  #0 'makeinlinelink :=     % state variable managed by setup.inlinelink
  "" 'openinlinelink :=     % ditto
  "" 'closeinlinelink :=    % ditto
}
INTEGERS { 
  bracket.state
  outside.brackets
  open.brackets
  within.brackets
  close.brackets
}
$mymarkerend
EOD
	$line = $_;
	until ($line =~ /\{.*\}.*\{/s) {
	    $line .= <IN>;
	}
	$line =~ s/(\{.*?\}.*?\{)/$1 #0 'outside.brackets := $mymarker
  #1 'open.brackets :=
  #2 'within.brackets :=
  #3 'close.brackets :=

 /s;
	print OUT $line;
	$found{initconsts} = 1;
	next;
    };

    /^ *EXECUTE *\{init\.state\.consts\}/ && do {
        print OUT "EXECUTE {init.urlbst.variables}\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{new.block\}/ && do {
        $found{newblock} = 1;
    };

    /^ *FUNCTION *{output\.nonnull}/ && do {
	print OUT "$mymarker\n";
	print OUT "FUNCTION {output.nonnull.original}\n";
        copy_block();
	print_output_functions();
	$found{outputnonnull} = 1;
	next;
    };

    /FUNCTION *\{fin.entry\}/ && do {
        # Rename fin.entry to fin.entry.original (wrapped below)
        s/fin.entry/fin.entry.original/;
        $found{finentry} = 1;
        print OUT;
        next;
    };

    /^ *FUNCTION *{format\.date}/ && do {
	$found{formatdate} = 1;
	print OUT;
	next;
    };

    /^ *FUNCTION *{format\.title}/ && do {
        # record that we found this
	$found{formattitle} = 1;
        print OUT;
	next;
    };

    /^ *format\.b?title/ && do {
        # interpolate a call to setup.inlinelink
        print OUT "  title empty\$ 'skip\$ 'setup\.inlinelink if\$ $mymarker\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{article\}/ && do {

	print_missing_functions();
	print_webpage_def();

	print OUT;
	$found{article} = 1;
	next;
    };

    /FUNCTION *\{output.bibitem\}/ && do {
        # Rename output.bibitem to output.bibitem.original (wrapped below)
        s/{output.bibitem\}/\{output.bibitem.original\}/;
 	$found{outputbibitem} = 1;
        print OUT;
        next;
    };

    print OUT;
};

if ($exitstatus == 0) {
    # Skip this if we've already reported an error -- it'll only be confusing
    foreach $k (keys %found) {
        if ($found{$k} == 0) {
            print STDERR "$progname: $infile: failed to find feature $k\n";
        }
    }
}

close (IN);
close (OUT);

exit $exitstatus;;






sub print_output_functions {
    print OUT "$mymarker...\n";

    print OUT <<'EOD';
% The following three functions are for handling inlinelink.  They wrap
% a block of text which is potentially output with write$ by multiple
% other functions, so we don't know the content a priori.
% They communicate between each other using the variables makeinlinelink
% (which is true if a link should be made), and closeinlinelink (which holds
% the string which should close any current link.  They can be called
% at any time, but start.inlinelink will be a no-op unless something has
% previously set makeinlinelink true, and the two ...end.inlinelink functions
% will only do their stuff if start.inlinelink has previously set
% closeinlinelink to be non-empty.
FUNCTION {setup.inlinelink}
{ makeinlinelink
    { hrefform #1 = % hypertex
        { "\special {html:<a href=" quote$ * url * quote$ * "> }{" * 'openinlinelink :=
          "\special {html:</a>}" 'closeinlinelink :=
          }
        { hrefform #2 = % hyperref
            { "\href{" url * "}{" * 'openinlinelink :=
              "}" 'closeinlinelink :=
              }
            'skip$
          if$ % hrefform #2 =
        }
      if$ % hrefform #1 =
      #0 'makeinlinelink :=
    }
    'skip$
 if$ % makeinlinelink
}
FUNCTION {add.inlinelink}
{ openinlinelink empty$
    'skip$
    { openinlinelink swap$ * closeinlinelink *
      "" 'openinlinelink :=
      }
  if$
}
EOD

    # new.block is defined elsewhere

    print OUT <<'EOD';
FUNCTION {output.nonnull}
{ % Save the thing we've been asked to output
  's :=
  % If the bracket-state is close.brackets, then add a close-bracket to
  % what is currently at the top of the stack, and set bracket.state
  % to outside.brackets
  bracket.state close.brackets =
    { "]" *
      outside.brackets 'bracket.state :=
    }
    'skip$
  if$
  bracket.state outside.brackets =
    { % We're outside all brackets -- this is the normal situation.
      % Write out what's currently at the top of the stack, using the
      % original output.nonnull function.
      s
      add.inlinelink
      output.nonnull.original % invoke the original output.nonnull
    }
    { % Still in brackets.  Add open-bracket or (continuation) comma, add the
      % new text (in s) to the top of the stack, and move to the close-brackets
      % state, ready for next time (unless inbrackets resets it).  If we come
      % into this branch, then output.state is carefully undisturbed.
      bracket.state open.brackets =
        { " [" * }
        { ", " * } % bracket.state will be within.brackets
      if$ 
      s * 
      close.brackets 'bracket.state :=
    }
  if$
}

% Call this function just before adding something which should be presented in 
% brackets.  bracket.state is handled specially within output.nonnull.
FUNCTION {inbrackets}
{ bracket.state close.brackets =
    { within.brackets 'bracket.state := } % reset the state: not open nor closed
    { open.brackets 'bracket.state := }
  if$
}

FUNCTION {format.lastchecked}
{ lastchecked empty$
    { "" }
    { inbrackets "cited " lastchecked * }
  if$
}
EOD
    print OUT "$mymarkerend\n";
}

sub print_webpage_def {
    print OUT "$mymarker...\n";

    # Some of the functions below call new.block, so we need a dummy
    # version, in the case where the style being edited doesn't supply
    # that function.
    if (! $found{newblock}) {
        print OUT "FUNCTION {new.block} % dummy new.block function\n{\n  % empty\n}\n\n";
        $found{newblock} = 1;
    }

    print OUT <<'EOD';
% Functions for making hypertext links.
% In all cases, the stack has (link-text href-url)
%
% make 'null' specials
FUNCTION {make.href.null}
{
  pop$
}
% make hypertex specials
FUNCTION {make.href.hypertex}
{ 
  "\special {html:<a href=" quote$ *
  swap$ * quote$ * "> }" * swap$ *
  "\special {html:</a>}" *
}
% make hyperref specials
FUNCTION {make.href.hyperref}
{ 
  "\href {" swap$ * "} {\path{" * swap$ * "}}" *
}
FUNCTION {make.href}
{ hrefform #2 =
    'make.href.hyperref      % hrefform = 2
    { hrefform #1 =
        'make.href.hypertex  % hrefform = 1
        'make.href.null      % hrefform = 0 (or anything else)
      if$
    }
  if$
}

% If inlinelinks is true, then format.url should be a no-op, since it's
% (a) redundant, and (b) could end up as a link-within-a-link.
FUNCTION {format.url}
{ inlinelinks #1 = url empty$ or
   { "" }
   { hrefform #1 =
       { % special case -- add HyperTeX specials
         urlintro "\url{" url * "}" * url make.href.hypertex * }
       { urlintro "\url{" * url * "}" * }
     if$
   }
  if$
}

FUNCTION {format.eprint}
{ eprint empty$
    { "" }
    { eprintprefix eprint * eprinturl eprint * make.href }
  if$
}

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { doiprefix doi * doiurl doi * make.href }
  if$
}

% Output a URL.  We can't use the more normal idiom (something like
% `format.url output'), because the `inbrackets' within
% format.lastchecked applies to everything between calls to `output',
% so that `format.url format.lastchecked * output' ends up with both
% the URL and the lastchecked in brackets.
FUNCTION {output.url}
{ url empty$
    'skip$ 
    { new.block 
      format.url output
      format.lastchecked output 
    }
  if$
}

FUNCTION {output.web.refs}
{
  new.block
  output.url
  addeprints eprint empty$ not and
    { format.eprint output.nonnull }
    'skip$
  if$
  adddoiresolver doi empty$ not and
    { format.doi output.nonnull }
    'skip$
  if$
}

% Wrapper for output.bibitem.original.
% If the URL field is not empty, set makeinlinelink to be true,
% so that an inline link will be started at the next opportunity
FUNCTION {output.bibitem}
{ outside.brackets 'bracket.state :=
  output.bibitem.original
  inlinelinks url empty$ not and
    { #1 'makeinlinelink := }
    { #0 'makeinlinelink := }
  if$
}

% Wrapper for fin.entry.original
FUNCTION {fin.entry}
{ output.web.refs  % urlbst
  makeinlinelink       % ooops, it appears we didn't have a title for inlinelink
    { setup.inlinelink % add some artificial link text here, as a fallback
      "[link]" output.nonnull }
    'skip$
  if$
  bracket.state close.brackets = % urlbst
    { "]" * }
    'skip$
  if$
  fin.entry.original
}

% Webpage entry type.
% Title and url fields required;
% author, note, year, month, and lastchecked fields optional
% See references 
%   ISO 690-2 http://www.nlc-bnc.ca/iso/tc46sc9/standard/690-2e.htm
%   http://www.classroom.net/classroom/CitingNetResources.html
%   http://neal.ctstateu.edu/history/cite.html
%   http://www.cas.usf.edu/english/walker/mla.html
% for citation formats for web pages.
FUNCTION {webpage}
{ output.bibitem
  author empty$
    { editor empty$
        'skip$  % author and editor both optional
        { format.editors output.nonnull }
      if$
    }
    { editor empty$
        { format.authors output.nonnull }
        { "can't use both author and editor fields in " cite$ * warning$ }
      if$
    }
  if$
  new.block
  title empty$ 'skip$ 'setup.inlinelink if$
  format.title "title" output.check
  inbrackets "online" output
  new.block
  year empty$
    'skip$
    { format.date "year" output.check }
  if$
  % We don't need to output the URL details ('lastchecked' and 'url'),
  % because fin.entry does that for us, using output.web.refs.  The only
  % reason we would want to put them here is if we were to decide that
  % they should go in front of the rather miscellaneous information in 'note'.
  new.block
  note output
  fin.entry
}
EOD

    print OUT "$mymarkerend\n\n\n";
}


sub print_missing_functions {
    # We've got to the bit of the file which handles the entry
    # types, so write out the webpage entry handler.  This uses
    # the format.date function, which which many but not all
    # bst files have (for example, apalike doesn't).  So
    # check that we either have found this function already, or
    # add it.
    if (! $found{formatdate}) {
	if ($found{entrymonth}) {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    { month empty$
	{ "" }
	{ "there's a month but no year in " cite$ * warning$
	  month
	}
      if$
    }
    { month empty$
	'year
	{ month " " * year * }
      if$
    }
  if$
}
EOD
	} else {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    'skip$
    { %write$
      "(" year * ")" *
    }
  if$
}
EOD
  	}
	$found{formatdate} = 1;
    }

    # If the style file didn't supply a format.title function, then supply
    # one here (the {webpage} function requires it).
    if (! $found{formattitle}) {
	print OUT <<'EOD';
FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}
EOD
    $found{formattitle} = 1;
    }
}

# Utility function: Keep track of open and close braces in the string argument.
# Keep state in $bracematchtotal, return the current value.
sub bracematcher {
    my $s = shift;
    $s =~ s/[^\{\}]//g;
    #print "s=$s\n";
    foreach my $c (split (//, $s)) {
	$bracematchtotal += ($c eq '{' ? 1 : -1);
    }
    return $bracematchtotal;
}

# Utility function: use bracematcher to copy the complete block which starts
# on or after the current line.
sub copy_block {
    $bracematchtotal = 0;
    # copy any leading lines which don't have braces (presumably comments)
    while (defined ($line = <IN>) && ($line !~ /{/)) {
        print OUT $line;
    }
    while (defined ($line) && bracematcher($line) > 0) {
        print OUT $line;
        $line = <IN>;
    }
    print OUT "$line\n";	# print out terminating \} (assumed
    				# alone on the line)
}


==> README <==
==========================================================================

The `caption' package bundle
Copyright (C) 1994-2013 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
http://sourceforge.net/projects/latex-caption/

If you need help for installation please visit:
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=inst-miktex*
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=installthings
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=privinst

If you need help using these packages please visit:
http://www.latex-community.org/
http://tex.stackexchange.com/
http://www.mrunix.de/            (German)
http://www.golatex.de/           (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please visit:
http://sourceforge.net/p/latex-caption/tickets/

--------------------------------------------------------------------------

The `caption' package v3.3 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.1 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.3 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.1 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

The `newfloat' package v1.1 offers the command \DeclareFloatingEnvironment
for defining new floating environments which behave like the existing
floating environments "figure" and "table".

User Manual: newfloat.pdf (English)

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)

